Mathematical Cookbook for Snapshot Compressive Imaging

The author intends to provide you with a beautiful, elegant, user-friendly cookbook for mathematics in Snapshot Compressive Imaging (SCI). Currently, the cookbook is composed of introduction, conventional optimization, and deep equilibrium models. The latest releases are strongly recommended! For any other questions, suggestions, or comments, feel free to email the author.

==> sections/dip.tex <==
\chapter{PnP + DIP: Solving Plug-and-Play Problem with Deep Image Prior}

\section{Review of DIP}

\section{Joint Framework}
